Probing surfactant bilayer interactions by tracking optically trapped single nanoparticles

Single-particle tracking and optical tweezers are powerful techniques for studying diverse processes at the microscopic scale. The stochastic behavior of a microscopically observable particle contains information about its interaction with surrounding molecules, and an optical tweezer can further facilitate this observation with its ability to constrain the particle to an area of interest. Although these techniques found their initial applications in biology, they can also shed new light on colloid and interface phenomena by unveiling nanoscale morphologies and molecular-level interactions in real time, which have been obscured in traditional ensemble analysis. Here we demonstrate the application of single-particle tracking and optical tweezers for studying molecular interactions at solid-liquid interfaces. Specifically, we investigate the behavior of surfactants at the water-glass interface by tracing their interactions with gold nanoparticles that are optically trapped on these molecules. We discover the underlying mechanisms governing the particle motion, which can be explained by hydrophobic interactions, disruptions, and rearrangements among surfactant monomers at the interfaces. Such interpretations are further supported by statistical analysis of an individual trajectory and comparison to theoretical predictions. Our findings provide new insights into the surfactant dynamics in this specific system but also illustrate the promise of single-particle tracking and optical manipulation in studying nanoscale physics and chemistry of surfaces and interfaces.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
